Differentiable DAG Sampling

We propose a new differentiable probabilistic model over DAGs (DP-DAG). DP-DAG allows fast and differentiable DAG sampling suited to continuous optimization. To this end, DP-DAG samples a DAG by successively (1) sampling a linear ordering of the node and (2) sampling edges consistent with the sampled linear ordering. We further propose VI-DP-DAG, a new method for DAG learning from observational data which combines DP-DAG with variational inference. Hence,VI-DP-DAG approximates the posterior probability over DAG edges given the observed data. VI-DP-DAG is guaranteed to output a valid DAG at any time during training and does not require any complex augmented Lagrangian optimization scheme in contrast to existing differentiable DAG learning approaches. In our extensive experiments, we compare VI-DP-DAG to other differentiable DAG learning baselines on synthetic and real datasets. VI-DP-DAG significantly improves DAG structure and causal mechanism learning while training faster than competitors.

==> tables/data_p100_e100_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &            \textbf{Un-AUC-PR} &           \textbf{Un-AUC-ROC} &           \textbf{Dir-AUC-PR} &          \textbf{Dir-AUC-ROC} \\
\midrule
    \textbf{DAG-GNN} &           $      7.46\pm0.24$ &           $     49.14\pm0.39$ &           $      2.85\pm0.16$ &           $     50.43\pm0.59$ \\
     \textbf{DAG-NF} &           $      2.12\pm0.03$ &           $     50.13\pm0.09$ &           $      1.10\pm0.02$ &           $     50.12\pm0.06$ \\
   \textbf{GraN-DAG} &           \underline{$     19.67\pm0.58$} &            \underline{$     64.47\pm0.5$} &           \underline{$     11.63\pm0.46$} &           \underline{$     60.49\pm0.38$} \\
 \textbf{Masked-DAG} &           $      8.78\pm0.31$ &           $     53.46\pm0.16$ &           $      7.41\pm0.32$ &           $     53.29\pm0.16$ \\
  \textbf{VI-DP-DAG} &  $\mathbf{     48.38}\pm0.88$ &  $\mathbf{     94.46}\pm0.16$ &  $\mathbf{     29.34}\pm0.93$ &  $\mathbf{     72.93}\pm0.55$ \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on ER-100-100 for all differentiable DAG learning models with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:er-100-100}
    \vspace{-3mm}
\end{table*}

==> tables/data_p100_e400_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &            \textbf{Un-AUC-PR} &           \textbf{Un-AUC-ROC} &           \textbf{Dir-AUC-PR} &          \textbf{Dir-AUC-ROC} \\
\midrule
    \textbf{DAG-GNN} &           \underline{$     14.65\pm0.25$} &            $     49.05\pm0.2$ &           \underline{$      5.56\pm0.09$} &           $     47.47\pm0.29$ \\
     \textbf{DAG-NF} &           $      7.82\pm0.04$ &           $     49.98\pm0.02$ &           $      3.94\pm0.02$ &           $     50.05\pm0.02$ \\
   \textbf{GraN-DAG} &           $      9.73\pm0.11$ &           \underline{$     52.82\pm0.11$} &           $      4.42\pm0.04$ &           \underline{$     51.04\pm0.06$} \\
 \textbf{Masked-DAG} &           $      8.93\pm0.12$ &           $     50.65\pm0.06$ &            $      4.73\pm0.1$ &           $     50.52\pm0.06$ \\
  \textbf{VI-DP-DAG} &  $\mathbf{     36.98}\pm0.98$ &  $\mathbf{     77.23}\pm0.63$ &  $\mathbf{     19.00}\pm1.07$ &  $\mathbf{     60.35}\pm1.01$ \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on ER-100-400 for all differentiable DAG learning models with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:er-100-400}
    \vspace{-3mm}
\end{table*}

==> tables/data_p10_e10_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &            \textbf{Un-AUC-PR} &           \textbf{Un-AUC-ROC} &           \textbf{Dir-AUC-PR} &          \textbf{Dir-AUC-ROC} \\
\midrule
    \textbf{DAG-GNN} &           $     44.20\pm1.66$ &           $     63.55\pm1.06$ &            $     18.35\pm0.9$ &            $     51.59\pm1.0$ \\
     \textbf{DAG-NF} &           $     28.22\pm0.88$ &           $     54.07\pm0.63$ &           $     19.47\pm0.88$ &           $     55.41\pm0.61$ \\
   \textbf{GraN-DAG} &  $\mathbf{     91.17}\pm0.69$ &  $\mathbf{     96.76}\pm0.29$ &  $\mathbf{     89.96}\pm0.69$ &  $\mathbf{     97.38}\pm0.25$ \\
 \textbf{Masked-DAG} &           $     44.74\pm1.77$ &           $     66.58\pm1.03$ &            $     30.23\pm1.8$ &           $     62.28\pm1.03$ \\
  \textbf{VI-DP-DAG} &           \underline{$     82.88\pm1.48$} &           \underline{$     95.00\pm0.51$} &           \underline{$     62.61\pm2.84$} &           \underline{$     83.27\pm1.36$} \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on ER-10-10 for all differentiable DAG learning models with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:er-10-10}
    \vspace{-3mm}
\end{table*}

==> tables/data_p10_e40_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &            \textbf{Un-AUC-PR} &           \textbf{Un-AUC-ROC} &           \textbf{Dir-AUC-PR} &          \textbf{Dir-AUC-ROC} \\
\midrule
    \textbf{DAG-GNN} &           $     85.31\pm0.53$ &           $     55.86\pm0.69$ &           $     49.26\pm0.79$ &           $     55.76\pm0.67$ \\
     \textbf{DAG-NF} &           $     83.46\pm0.29$ &           $     56.72\pm0.43$ &           $     42.86\pm0.23$ &           $     51.93\pm0.43$ \\
   \textbf{GraN-DAG} &  $\mathbf{     96.47}\pm0.14$ &  $\mathbf{     89.20}\pm0.38$ &  $\mathbf{     93.54}\pm0.39$ &  $\mathbf{     95.26}\pm0.34$ \\
 \textbf{Masked-DAG} &            $     84.05\pm0.3$ &           $     58.94\pm0.31$ &           $     48.92\pm0.42$ &           $     57.19\pm0.35$ \\
  \textbf{VI-DP-DAG} &            \underline{$     94.59\pm0.5$} &           \underline{$     86.09\pm1.07$} &           \underline{$     79.42\pm0.97$} &           \underline{$     83.93\pm0.76$} \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on ER-10-40 for all differentiable DAG learning models with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:er-10-40}
    \vspace{-3mm}
\end{table*}

==> tables/data_p50_e200_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &            \textbf{Un-AUC-PR} &           \textbf{Un-AUC-ROC} &           \textbf{Dir-AUC-PR} &          \textbf{Dir-AUC-ROC} \\
\midrule
    \textbf{DAG-GNN} &           $     18.67\pm0.17$ &           $     48.44\pm0.15$ &           $      8.21\pm0.15$ &           $     47.83\pm0.34$ \\
     \textbf{DAG-NF} &           $     16.11\pm0.12$ &           $     50.20\pm0.03$ &           $      8.15\pm0.07$ &           $     50.19\pm0.02$ \\
   \textbf{GraN-DAG} &            \underline{$     25.11\pm0.4$} &           \underline{$     56.57\pm0.35$} &           \underline{$     17.61\pm0.47$} &           \underline{$     56.35\pm0.34$} \\
 \textbf{Masked-DAG} &           $     17.55\pm0.14$ &           $     51.09\pm0.05$ &           $      9.14\pm0.09$ &           $     50.81\pm0.04$ \\
  \textbf{VI-DP-DAG} &  $\mathbf{     62.08}\pm0.34$ &  $\mathbf{     84.53}\pm0.25$ &  $\mathbf{     41.70}\pm0.39$ &  $\mathbf{     71.08}\pm0.33$ \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on ER-50-200 for all differentiable DAG learning models with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:er-50-200}
    \vspace{-3mm}
\end{table*}

==> tables/data_p50_e50_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &           \textbf{Un-AUC-PR} &           \textbf{Un-AUC-ROC} &           \textbf{Dir-AUC-PR} &          \textbf{Dir-AUC-ROC} \\
\midrule
    \textbf{DAG-GNN} &          $     16.20\pm1.03$ &           $     52.20\pm0.78$ &           $      5.52\pm0.33$ &            $     51.80\pm0.6$ \\
     \textbf{DAG-NF} &          $      4.48\pm0.13$ &           $     50.32\pm0.08$ &           $      2.35\pm0.09$ &           $     50.22\pm0.05$ \\
   \textbf{GraN-DAG} &           \underline{$     42.97\pm1.1$} &            \underline{$     71.40\pm0.7$} &           \underline{$     38.07\pm0.97$} &           \underline{$     70.27\pm0.65$} \\
 \textbf{Masked-DAG} &          $     11.29\pm0.46$ &           $     53.97\pm0.24$ &            $      7.66\pm0.4$ &           $     53.26\pm0.22$ \\
  \textbf{VI-DP-DAG} &  $\mathbf{     75.70}\pm0.8$ &  $\mathbf{     97.26}\pm0.12$ &  $\mathbf{     52.95}\pm0.95$ &  $\mathbf{     80.85}\pm0.46$ \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on ER-50-50 for all differentiable DAG learning models with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:er-50-50}
    \vspace{-3mm}
\end{table*}

==> tables/data_sf_p10_e10_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &            \textbf{Un-AUC-PR} &           \textbf{Un-AUC-ROC} &           \textbf{Dir-AUC-PR} &          \textbf{Dir-AUC-ROC} \\
\midrule
    \textbf{DAG-GNN} &           $     38.91\pm1.56$ &           $     46.56\pm1.56$ &           $     20.04\pm0.62$ &           $     49.83\pm0.63$ \\
     \textbf{DAG-NF} &           $     24.03\pm0.87$ &           $     51.38\pm0.81$ &           $     11.78\pm0.46$ &           $     50.93\pm0.39$ \\
   \textbf{GraN-DAG} &  $\mathbf{     93.14}\pm0.75$ &  $\mathbf{     97.59}\pm0.28$ &  $\mathbf{     93.01}\pm0.77$ &  $\mathbf{     98.85}\pm0.14$ \\
 \textbf{Masked-DAG} &           $     48.96\pm1.79$ &           $     69.21\pm1.05$ &           $     39.42\pm2.22$ &            $     66.92\pm1.2$ \\
  \textbf{VI-DP-DAG} &           \underline{$     77.26\pm0.97$} &            \underline{$     93.47\pm0.4$} &           \underline{$     66.35\pm1.69$} &           \underline{$     87.05\pm1.18$} \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on SF-10-40 for all differentiable DAG learning models with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:sf-10-40}
    \vspace{-3mm}
\end{table*}

==> tables/data_sf_p50_e200_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &            \textbf{Un-AUC-PR} &           \textbf{Un-AUC-ROC} &           \textbf{Dir-AUC-PR} &          \textbf{Dir-AUC-ROC} \\
\midrule
    \textbf{DAG-GNN} &           $     14.94\pm0.17$ &           $     51.41\pm0.26$ &           $      6.91\pm0.12$ &           $     50.31\pm0.27$ \\
     \textbf{DAG-NF} &            $     11.83\pm0.1$ &           $     50.18\pm0.03$ &           $      5.86\pm0.06$ &           $     50.02\pm0.02$ \\
   \textbf{GraN-DAG} &           \underline{$     18.75\pm0.29$} &           \underline{$     54.76\pm0.17$} &           \underline{$     12.35\pm0.32$} &           \underline{$     53.31\pm0.43$} \\
 \textbf{Masked-DAG} &           $     14.39\pm0.13$ &           $     51.64\pm0.06$ &           $      7.23\pm0.12$ &           $     50.97\pm0.06$ \\
  \textbf{VI-DP-DAG} &  $\mathbf{     33.81}\pm0.39$ &  $\mathbf{     68.18}\pm0.39$ &  $\mathbf{     17.46}\pm0.34$ &  $\mathbf{     59.70}\pm0.65$ \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on SF-50-200 for all differentiable DAG learning models with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:sf-50-200}
    \vspace{-3mm}
\end{table*}

==> tables/data_sf_p50_e50_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &           \textbf{Un-AUC-PR} &           \textbf{Un-AUC-ROC} &           \textbf{Dir-AUC-PR} &          \textbf{Dir-AUC-ROC} \\
\midrule
    \textbf{DAG-GNN} &          $      7.76\pm0.26$ &           $     49.24\pm0.58$ &           $      3.36\pm0.14$ &           $     49.66\pm0.52$ \\
     \textbf{DAG-NF} &           $      3.92\pm0.0$ &            $     49.83\pm0.0$ &            $      1.96\pm0.0$ &            $     49.92\pm0.0$ \\
   \textbf{GraN-DAG} &          \underline{$     21.82\pm0.64$} &           \underline{$     64.16\pm0.51$} &           \underline{$     18.12\pm0.66$} &  $\mathbf{     62.78}\pm0.47$ \\
 \textbf{Masked-DAG} &          $     10.39\pm0.23$ &           $     53.37\pm0.12$ &           $      6.11\pm0.22$ &            $     52.33\pm0.1$ \\
  \textbf{VI-DP-DAG} &  $\mathbf{     46.67}\pm0.8$ &  $\mathbf{     80.50}\pm0.49$ &  $\mathbf{     23.25}\pm0.89$ &            \underline{$     60.74\pm0.7$} \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on SF-50-50 for all differentiable DAG learning models with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:sf-50-50}
    \vspace{-3mm}
\end{table*}

==> tables/proc_data_p100_e100_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &          \textbf{Un-AUC-PR*} &         \textbf{Un-AUC-ROC*} &          \textbf{Dir-AUC-PR*} &        \textbf{Dir-AUC-ROC*} \\
\midrule
        \textbf{CAM} &  $\mathbf{     82.17}\pm0.0$ &  $\mathbf{     95.40}\pm0.0$ &            \underline{$     75.07\pm0.0$} &  $\mathbf{     93.43}\pm0.0$ \\
   \textbf{GraN-DAG} &          $     77.87\pm0.47$ &          $     90.08\pm0.28$ &  $\mathbf{     76.61}\pm0.53$ &          \underline{$     89.71\pm0.29$} \\
 \textbf{Masked-DAG} &          $      8.78\pm0.31$ &          $     53.46\pm0.16$ &           $      7.41\pm0.32$ &          $     53.29\pm0.16$ \\
  \textbf{VI-DP-DAG} &          \underline{$     79.39\pm0.57$} &          \underline{$     93.78\pm0.21$} &           $     46.11\pm1.13$ &          $     80.34\pm0.37$ \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on ER-100-100 for all DAG learning models with non-differentiable processing with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:proc-er-100-100}
    \vspace{-0mm}
\end{table*}

==> tables/proc_data_p100_e400_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &          \textbf{Un-AUC-PR*} &         \textbf{Un-AUC-ROC*} &         \textbf{Dir-AUC-PR*} &        \textbf{Dir-AUC-ROC*} \\
\midrule
        \textbf{CAM} &  $\mathbf{     56.00}\pm0.0$ &  $\mathbf{     79.46}\pm0.0$ &  $\mathbf{     49.97}\pm0.0$ &  $\mathbf{     78.24}\pm0.0$ \\
   \textbf{GraN-DAG} &          $     38.28\pm0.39$ &          $     66.95\pm0.24$ &           \underline{$     35.39\pm0.4$} &          \underline{$     66.85\pm0.24$} \\
 \textbf{Masked-DAG} &          $      9.03\pm0.12$ &          $     50.72\pm0.06$ &           $      4.76\pm0.1$ &          $     50.55\pm0.06$ \\
  \textbf{VI-DP-DAG} &          \underline{$     44.45\pm0.61$} &          \underline{$     72.71\pm0.23$} &          $     22.32\pm0.93$ &          $     64.57\pm0.39$ \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on ER-100-400 for all DAG learning models with non-differentiable processing with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:proc-er-100-400}
    \vspace{-0mm}
\end{table*}

==> tables/proc_data_p10_e10_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &          \textbf{Un-AUC-PR*} &         \textbf{Un-AUC-ROC*} &         \textbf{Dir-AUC-PR*} &        \textbf{Dir-AUC-ROC*} \\
\midrule
        \textbf{CAM} &  $\mathbf{    100.00}\pm0.0$ &  $\mathbf{    100.00}\pm0.0$ &  $\mathbf{    100.00}\pm0.0$ &  $\mathbf{    100.00}\pm0.0$ \\
   \textbf{GraN-DAG} &          \underline{$     94.80\pm0.76$} &          \underline{$     98.68\pm0.22$} &          \underline{$     86.34\pm1.92$} &          \underline{$     95.96\pm0.55$} \\
 \textbf{Masked-DAG} &          $     45.56\pm1.64$ &          $     66.35\pm1.02$ &          $     29.69\pm1.78$ &           $     61.96\pm1.0$ \\
  \textbf{VI-DP-DAG} &          $     88.17\pm1.07$ &          $     96.18\pm0.43$ &          $     66.17\pm2.66$ &           $     87.58\pm1.0$ \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on ER-10-10 for all DAG learning models with non-differentiable processing with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:proc-er-10-10}
    \vspace{-0mm}
\end{table*}

==> tables/proc_data_p10_e40_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &           \textbf{Un-AUC-PR*} &          \textbf{Un-AUC-ROC*} &          \textbf{Dir-AUC-PR*} &         \textbf{Dir-AUC-ROC*} \\
\midrule
        \textbf{CAM} &            $     89.56\pm0.0$ &            $     78.09\pm0.0$ &            \underline{$     79.56\pm0.0$} &            \underline{$     85.54\pm0.0$} \\
   \textbf{GraN-DAG} &  $\mathbf{     93.79}\pm0.38$ &  $\mathbf{     84.43}\pm0.78$ &  $\mathbf{     86.00}\pm0.55$ &  $\mathbf{     89.28}\pm0.37$ \\
 \textbf{Masked-DAG} &           $     84.00\pm0.31$ &           $     58.82\pm0.32$ &           $     48.77\pm0.43$ &           $     57.06\pm0.36$ \\
  \textbf{VI-DP-DAG} &           \underline{$     93.23\pm0.46$} &           \underline{$     83.11\pm0.92$} &           $     75.98\pm0.83$ &           $     80.75\pm0.62$ \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on ER-10-40 for all DAG learning models with non-differentiable processing with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:proc-er-10-40}
    \vspace{-0mm}
\end{table*}

==> tables/proc_data_p50_e200_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &           \textbf{Un-AUC-PR*} &          \textbf{Un-AUC-ROC*} &          \textbf{Dir-AUC-PR*} &         \textbf{Dir-AUC-ROC*} \\
\midrule
        \textbf{CAM} &           $     49.35\pm0.05$ &  $\mathbf{     74.45}\pm0.04$ &           \underline{$     41.35\pm0.06$} &  $\mathbf{     73.60}\pm0.04$ \\
   \textbf{GraN-DAG} &           \underline{$     49.85\pm0.66$} &           $     70.91\pm0.44$ &  $\mathbf{     44.78}\pm0.74$ &           \underline{$     70.78\pm0.44$} \\
 \textbf{Masked-DAG} &           $     17.55\pm0.14$ &           $     51.09\pm0.05$ &           $      9.14\pm0.09$ &           $     50.81\pm0.04$ \\
  \textbf{VI-DP-DAG} &  $\mathbf{     53.77}\pm0.36$ &           \underline{$     73.25\pm0.25$} &           $     36.54\pm0.34$ &            $     68.08\pm0.2$ \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on ER-50-200 for all DAG learning models with non-differentiable processing with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:proc-er-50-200}
    \vspace{-0mm}
\end{table*}

==> tables/proc_data_p50_e50_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &           \textbf{Un-AUC-PR*} &         \textbf{Un-AUC-ROC*} &          \textbf{Dir-AUC-PR*} &        \textbf{Dir-AUC-ROC*} \\
\midrule
        \textbf{CAM} &  $\mathbf{     92.60}\pm0.17$ &  $\mathbf{     98.89}\pm0.0$ &  $\mathbf{     92.56}\pm0.17$ &  $\mathbf{     98.96}\pm0.0$ \\
   \textbf{GraN-DAG} &           $     87.45\pm0.76$ &           $     93.51\pm0.4$ &           \underline{$     86.63\pm0.81$} &          \underline{$     93.25\pm0.41$} \\
 \textbf{Masked-DAG} &           $     11.34\pm0.45$ &          $     53.97\pm0.24$ &            $      7.71\pm0.4$ &          $     53.27\pm0.22$ \\
  \textbf{VI-DP-DAG} &           \underline{$     90.28\pm0.46$} &          \underline{$     95.93\pm0.24$} &           $     61.13\pm0.87$ &          $     85.21\pm0.38$ \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on ER-50-50 for all DAG learning models with non-differentiable processing with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:proc-er-50-50}
    \vspace{-0mm}
\end{table*}

==> tables/proc_data_sf_p10_e10_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &          \textbf{Un-AUC-PR*} &         \textbf{Un-AUC-ROC*} &         \textbf{Dir-AUC-PR*} &        \textbf{Dir-AUC-ROC*} \\
\midrule
        \textbf{CAM} &  $\mathbf{    100.00}\pm0.0$ &  $\mathbf{    100.00}\pm0.0$ &  $\mathbf{    100.00}\pm0.0$ &  $\mathbf{    100.00}\pm0.0$ \\
   \textbf{GraN-DAG} &          \underline{$     90.89\pm1.15$} &           \underline{$     94.44\pm0.7$} &          \underline{$     86.85\pm1.36$} &          \underline{$     93.79\pm0.68$} \\
 \textbf{Masked-DAG} &          $     48.07\pm1.63$ &           $     68.25\pm1.0$ &          $     38.96\pm1.99$ &           $     66.48\pm1.1$ \\
  \textbf{VI-DP-DAG} &          $     83.76\pm0.89$ &          $     90.65\pm0.52$ &          $     71.25\pm1.65$ &          $     85.52\pm0.81$ \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on SF-10-40 for all DAG learning models with non-differentiable processing with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:proc-sf-10-40}
    \vspace{-0mm}
\end{table*}

==> tables/proc_data_sf_p50_e200_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &           \textbf{Un-AUC-PR*} &          \textbf{Un-AUC-ROC*} &          \textbf{Dir-AUC-PR*} &         \textbf{Dir-AUC-ROC*} \\
\midrule
        \textbf{CAM} &  $\mathbf{     32.45}\pm0.13$ &  $\mathbf{     63.10}\pm0.04$ &  $\mathbf{     28.45}\pm0.13$ &  $\mathbf{     63.17}\pm0.04$ \\
   \textbf{GraN-DAG} &           $     29.28\pm0.41$ &           $     60.11\pm0.24$ &           \underline{$     24.74\pm0.44$} &           \underline{$     60.12\pm0.24$} \\
 \textbf{Masked-DAG} &           $     14.39\pm0.13$ &           $     51.64\pm0.06$ &           $      7.23\pm0.12$ &           $     50.97\pm0.06$ \\
  \textbf{VI-DP-DAG} &           \underline{$     30.17\pm0.29$} &           \underline{$     60.85\pm0.17$} &           $     15.78\pm0.29$ &           $     57.04\pm0.17$ \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on SF-50-200 for all DAG learning models with non-differentiable processing with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:proc-sf-50-200}
    \vspace{-0mm}
\end{table*}

==> tables/proc_data_sf_p50_e50_n1000_GP.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &           \textbf{Un-AUC-PR*} &         \textbf{Un-AUC-ROC*} &          \textbf{Dir-AUC-PR*} &        \textbf{Dir-AUC-ROC*} \\
\midrule
        \textbf{CAM} &  $\mathbf{     53.66}\pm0.16$ &  $\mathbf{     79.43}\pm0.0$ &  $\mathbf{     52.86}\pm0.16$ &  $\mathbf{     79.51}\pm0.0$ \\
   \textbf{GraN-DAG} &           $     49.86\pm0.99$ &          $     73.96\pm0.52$ &           \underline{$     47.71\pm0.99$} &           \underline{$     73.46\pm0.5$} \\
 \textbf{Masked-DAG} &           $     10.39\pm0.23$ &          $     53.37\pm0.12$ &           $      6.11\pm0.22$ &           $     52.33\pm0.1$ \\
  \textbf{VI-DP-DAG} &           \underline{$     50.56\pm0.96$} &          \underline{$     74.78\pm0.52$} &           $     25.41\pm0.97$ &          $     65.99\pm0.54$ \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on SF-50-50 for all DAG learning models with non-differentiable processing with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:proc-sf-50-50}
    \vspace{-0mm}
\end{table*}

==> tables/proc_sachs.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &          \textbf{Un-AUC-PR*} &          \textbf{Un-AUC-ROC*} &          \textbf{Dir-AUC-PR*} &         \textbf{Dir-AUC-ROC*} \\
\midrule
        \textbf{CAM} &          $     32.62\pm0.04$ &           $     55.07\pm0.06$ &           \underline{$     18.69\pm0.03$} &  $\mathbf{     56.98}\pm0.02$ \\
   \textbf{GraN-DAG} &           $     30.79\pm0.2$ &           $     52.07\pm0.21$ &            $     16.38\pm0.2$ &           $     52.22\pm0.26$ \\
 \textbf{Masked-DAG} &          \underline{$     36.98\pm0.25$} &           \underline{$     55.13\pm0.15$} &           $     17.74\pm0.31$ &           $     51.71\pm0.23$ \\
  \textbf{VI-DP-DAG} &  $\mathbf{     40.29}\pm0.4$ &  $\mathbf{     59.00}\pm0.06$ &  $\mathbf{     19.11}\pm0.44$ &           \underline{$     54.30\pm0.33$} \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on Sachs dataset for all DAG learning models with non-differentiable processing with AUC-PR and AUC-ROC scores with non-differentiable pre- and post-processing. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:proc-sachs}
    \vspace{-0mm}
\end{table*}

==> tables/proc_syntren.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &           \textbf{Un-AUC-PR*} &          \textbf{Un-AUC-ROC*} &          \textbf{Dir-AUC-PR*} &         \textbf{Dir-AUC-ROC*} \\
\midrule
        \textbf{CAM} &           \underline{$     18.27\pm0.03$} &           \underline{$     63.16\pm0.03$} &           $      7.57\pm0.01$ &           \underline{$     56.16\pm0.01$} \\
   \textbf{GraN-DAG} &           $     16.30\pm0.34$ &           $     54.91\pm0.21$ &           \underline{$      9.55\pm0.24$} &           $     53.77\pm0.19$ \\
 \textbf{Masked-DAG} &            $     17.24\pm0.4$ &           $     54.22\pm0.32$ &           $      8.78\pm0.42$ &           $     52.63\pm0.38$ \\
  \textbf{VI-DP-DAG} &  $\mathbf{     35.11}\pm0.91$ &  $\mathbf{     76.23}\pm0.68$ &  $\mathbf{     17.84}\pm0.98$ &  $\mathbf{     64.32}\pm1.05$ \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on Syntren dataset for all differentiable DAG learning models with non-differentiable processing with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:proc-syntren}
    \vspace{-0mm}
\end{table*}

==> tables/sachs.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &            \textbf{Un-AUC-PR} &           \textbf{Un-AUC-ROC} &           \textbf{Dir-AUC-PR} &          \textbf{Dir-AUC-ROC} \\
\midrule
    \textbf{DAG-GNN} &  $\mathbf{     49.92}\pm0.46$ &           \underline{$     59.59\pm0.57$} &  $\mathbf{     23.84}\pm0.52$ &           $     51.67\pm0.62$ \\
     \textbf{DAG-NF} &           $     35.66\pm0.32$ &           $     53.57\pm0.44$ &           $     15.43\pm0.11$ &           $     50.16\pm0.31$ \\
   \textbf{GraN-DAG} &           $     34.28\pm0.32$ &           $     54.57\pm0.36$ &           $     19.95\pm0.35$ &           \underline{$     55.91\pm0.33$} \\
 \textbf{Masked-DAG} &           $     36.98\pm0.25$ &           $     55.13\pm0.15$ &           $     17.74\pm0.31$ &           $     51.71\pm0.23$ \\
  \textbf{VI-DP-DAG} &           \underline{$     43.37\pm0.55$} &  $\mathbf{     59.78}\pm0.62$ &           \underline{$     22.96\pm0.81$} &  $\mathbf{     60.02}\pm0.91$ \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on Sachs dataset for all differentiable DAG learning models with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:sachs}
    \vspace{-3mm}
\end{table*}

==> tables/syntren.tex <==
\begin{table*}[!h]
    \centering
    %\tiny
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
     \textbf{Models} &            \textbf{Un-AUC-PR} &           \textbf{Un-AUC-ROC} &           \textbf{Dir-AUC-PR} &          \textbf{Dir-AUC-ROC} \\
\midrule
    \textbf{DAG-GNN} &           \underline{$     24.83\pm0.19$} &            \underline{$     66.75\pm0.2$} &           $      9.26\pm0.11$ &           $     59.61\pm0.19$ \\
     \textbf{DAG-NF} &           $     12.89\pm0.15$ &           $     49.02\pm0.24$ &           $      6.63\pm0.15$ &           $     49.11\pm0.16$ \\
   \textbf{GraN-DAG} &            $     19.89\pm0.4$ &           $     62.29\pm0.31$ &  $\mathbf{     15.39}\pm0.44$ &  $\mathbf{     63.91}\pm0.34$ \\
 \textbf{Masked-DAG} &           $     16.66\pm0.38$ &           $     53.93\pm0.28$ &           $      7.99\pm0.29$ &           $     52.26\pm0.35$ \\
  \textbf{VI-DP-DAG} &  $\mathbf{     26.33}\pm0.56$ &  $\mathbf{     70.84}\pm0.45$ &           \underline{$     14.17\pm0.76$} &           \underline{$     59.84\pm1.46$} \\
\bottomrule
\end{tabular}
    }
    \caption{DAG structure learning results on SynTReN dataset for all differentiable DAG learning models with AUC-PR and AUC-ROC scores. \emph{Un.} and \emph{Dir.} indicate scores for undirected and directed edges. Best scores among all models are in bold. Second best scores among all models are underlined.}
    \label{tab:syntren}
    \vspace{-3mm}
\end{table*}
